Predictive Modeling of Anatomy with Genetic and Clinical Data

We present a semi-parametric generative model for predicting anatomy of a patient in subsequent scans following a single baseline image. Such predictive modeling promises to facilitate novel analyses in both voxel-level studies and longitudinal biomarker evaluation. We capture anatomical change through a combination of population-wide regression and a non-parametric model of the subject's health based on individual genetic and clinical indicators. In contrast to classical correlation and longitudinal analysis, we focus on predicting new observations from a single subject observation. We demonstrate prediction of follow-up anatomical scans in the ADNI cohort, and illustrate a novel analysis approach that compares a patient's scans to the predicted subject-specific healthy anatomical trajectory. The code is available at https://github.com/adalca/voxelorb.

==> MICCAI2015 - arxiv2020/conclusion.tex <==
\section{Conclusions}
%Validation shows the method works, and the new application shows the interesting type of novel analyses possible. This type of prediction opens a world of opportunities. Future expansions of the model (better Ks, appearance model, etc.) will allow even more powerful analyses. E.G. developmental conditions, degenerative conditions (HD), etc.
%
%? Note the similarity to population imputation. 
%

We present a model to predict the anatomy in patient follow-up
images given just a baseline image using population trends and subject-specific genetic and
clinical information. We validate our prediction method on scalar volumes
and anatomical images, and show that it can be used as a powerful
tool to illustrate how a subject-specific brain might differ if it
were healthy. Through this and other new applications, our prediction
method presents a novel opportunity for the study of disease and
anatomical development.





==> MICCAI2015 - arxiv2020/experiments.tex <==
\section{Experiments}
\begin{figure}[t]
\centering
\includegraphics[width=0.97\linewidth]{./figures/exp1_prettyfigure_2_updated}
\caption{\footnotesize Relative error (lower is better) of volume prediction for seven structures for subjects in the top decile of volume change. 
	%For intracranial volume, whole brain volume, ventricles, hippocampus, entorhinal cortex, fusiform gyrus, and middle temporal gyrus, 
We report relative change between the baseline and the follow-up measurement (red), relative error in prediction using a population model (green), and the complete model (blue).}
\label{fig:volumeerror}
\end{figure}


\begin{figure}[b]
	\centering
	\includegraphics[width=0.97\linewidth]{figures/example_images}
	\caption{Example predicted volume, in axial, sagittal and coronal views. Qualitatively, the scan presents plausible anatomy, and would be challenging to discern from an actual scan.}
	\label{fig:examplesynthesis}
\end{figure}



\begin{figure}[tb]
	\centering
	\includegraphics[width=0.97\linewidth]{figures/exp2_prettyfigure_2_updated}
	\caption{Prediction results. Dice scores of labels propagated through three methods for several structures implicatd in AD in subjects with the most volume change for each structure. We report the prediction based on the registration of the actual follow-up scan to the atlas as an upper bound for warp-based prediction accuracy (black), predictions based on the population-wide linear regression model (green), and the full model (blue).} 
	\label{fig:ADDice}
\end{figure}





We illustrate our approach by predicting image-based phenotypes based
on genetic, clinical and imaging data in the ADNI longitudinal
study~\cite{jack2008}
%\footnote{AD Big Data DREAM Challenge: https://www.synapse.org/\#!Synapse:syn2290704} 
that includes two to
ten follow-up scans acquired~$0.5 - 7$ years after the baseline scan.  We use affine registration to align all subjects to
a template constructed from~$145$ randomly chosen subjects, and
compute non-linear registration warps~$\Phi_{AI}$ for each image using
ANTs~\cite{avants2011}. We utilize a list of~$21$ genetic loci
associated with Alzheimer's disease (AD) as the genetic vector $g$, and the 
standard clinical factors including age, gender, marital status,
education, disease diagnostic, and cognitive tests, as the clinical
indicator vector $c$. We learn the model parameters from 341 randomly chosen subjects
and predict follow-up volumes on a separate set of 100 subjects. To
evaluate the advantages of the proposed predictive model, we compare
its performance to a population-wide linear regression model that
ignores the subject-specific health profiles (i.e.,~$H=0$).

\subsection{Volumetric Predictions}

In the first simplified experiment, we define phenotype $y$ to be a
vector of several scalar volume measurements obtained using
FreeSurfer~\cite{fischl2012}. 
%{\color{red}These include intracranial volume, whole
%brain volume, ventricles, hippocampus, entorhinal cortex, fusiform
%gyrus, and middle temporal gyrus.} 
In addition to the population-wide
linear regression model, we include a simple approach of using the
baseline volume measurements as a predictor of the phenotype trajectory, effectively assuming no volume change with
time. Since in many subjects, the volume differences are
small, all three methods perform comparably when
evaluated on the whole test set. To evaluate the differences between
the methods, we focus on the subset of subjects with substantial
volume changes, reported in Fig.~\ref{fig:volumeerror}. 
Our method consistently achieves smaller relative errors than the
two baseline approaches.




% We also make use of pre-computed structure volumes for the ventricles,
% hippocampus, whole brain volume, entorhinal cortex, fusiform gyrus,
% middle temporal gyrus and intercranial volume using
% FreeSurfer~\cite{fischl2012}.  In our first experiment, we predict
% volume measurements of the available anatomical structures mentioned
% above. We use our prediction method, as well as a simple linear
% regression model that does not consider subject-specific health
% profiles (i.e,~$H=0$). Our model is able to accurately predict
% volumetric changes. Many subjects do not have dramatic changes in the
% given structures over time, and our algorithm shows modest improvement
% over linear regression with an average of~$0.126$ points less percent
% error. However, when considering the more difficult case of prediction
% of subjects with large volume changes over time, our model improves
% prediction dramatically as shown in Fig.~\ref{fig:volumeerror}.


\subsection{Anatomical Prediction}


%\begin{figure}[t]
%\centering
%\includegraphics[width=0.71\linewidth]{./figures/exp2_prettyfigure2}
%\includegraphics[width=0.233\linewidth]{./figures/healthyprediction_135299}
%\includegraphics[width=0.037\linewidth]{./figures/colorbar}
%\caption{\footnotesize Prediction results. Left: Dice scores of labels propagated through three methods for several structures implicatd in AD in subjects with the most volume change for each structure. We report the prediction based on the registration of the actual follow-up scan to the atlas as an upper bound for warp-based prediction accuracy (red), predictions based on the population-wide linear regression model (green), and the full model (blue). Right: A predicted anatomical image for a patient diagnosed with AD using a healthy model. The color overlay shows the squared magnitude of the difference in predicted versus observed deformations, indicating a significantly different expansion trajectory of the ventricles.} %when compared to the observed follow-up.
%\label{fig:ADDice}
%\end{figure}


We also evaluate the model for full anatomical scan prediction. An example prediction is shown in Fig.~\ref{fig:examplesynthesis}. To quantify prediction accuracy, we propagate segmentation labels of
relevant anatomical structures from the baseline scan to the predicted
scan using the predicted warps. We compare the predicted
segmentation label maps with the actual segmentations of the follow-up
scans. The warps computed based on the actual follow-up
scans through the atlas provide an indication of the best accuracy the predictive model
could achieve when using warps to represent images. Similar to the
volumetric predictions, the full model offers modest improvements when
evaluated on the entire test set, and substantial improvements in 
segmentation accuracy when evaluated in the subjects who exhibit large
volume changes between the baseline scan and the follow-up scan, as
reported in Fig.~\ref{fig:ADDice} and exemplified in Fig.~\ref{fig:comparisoneg}.
In both experiments, all components~$h_g, h_c$ and~$h_I$ contributed significantly to the improved predictions.

\begin{figure}[t]
	\centering
	\includegraphics[width=0.97\linewidth]{figures/comparison_example}
	\caption{Example comparison of predicted follow-up scans. This subjects presents with significant ventricle expansion due to brain atrophy from the baseline image to the follow-up observation. The predicted scan using the full model is able to capture significantly more of the ventricle expansion compared to the age-regression based follow-up. Qualitatively, both predicted follow-up scans present as plausible anatomical images. 
		%\todo{Choose a more illustrative subject.}
	}
	\label{fig:comparisoneg}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{figures/exp2example}
	%\includegraphics[width=0.233\linewidth]{\figdir/healthyprediction_135299}
	\includegraphics[width=0.052\linewidth]{figures/colorbar}
	\caption{Comparison of an acquired and predicted anatomical image for a patient diagnosed with AD using a healthy model. Ventricles are outlines in red. The third image shows the predicted follow-up with a color overlay, indicating the squared magnitude of the difference in predicted versus observed deformation field, showing that the ventricles expand significantly less in the predicted scan. The figures indicate a significantly different expansion trajectory of the ventricles when compared to the observed follow-up.} 
	\label{fig:exampleADNI}
\end{figure}

Our experimental results suggest that the anatomical model depends on
registration accuracy.  In particular, we observe that directly
registering the follow-up scan to the baseline scan leads to better
alignment of segmentation labels than when transferring the labels
through a composition of the transformations from the scans to the
atlas space. This suggests that a different choice of appearance model
may improve prediction accuracy, a promising direction for future
work.




\subsection{Example Application}


To demonstrate the potential of the anatomical prediction, we predict
the follow-up scan of a patient diagnosed with dementia as if the
patient were healthy. Specifically, we train our model using healthy
subjects, and predict follow-up scans for AD patients.  In
Fig.~\ref{fig:exampleADNI} we illustrate an example result, comparing
the areas of brain anatomy that differ from the observed follow-up in the predicted
\textit{healthy} brain of this AD patient. Our prediction indicates that
ventricle expansion would be different if this patient had a healthy
trajectory.











%\begin{figure}[t]
%\centering
%\includegraphics[width=0.29\linewidth]{./figures/healthyprediction_135299}
%\includegraphics[width=0.69\linewidth]{./figures/patientdiff}
%\caption{Comparison of actual follow-ups compared to predicted images from model parameters trained on healthy images. On the left, we overlap the difference in predicted and actual follow-up warps overlayed over the predicted image, illustrating significant differences in the ventricles and cortex. On the right,}
%\label{fig:application}
%\end{figure}

%\begin{figure}[t]
%\centering
%\begin{minipage}[t]{0.49\linewidth}
%\includegraphics[width=1\linewidth]{./figures/patientdiff}
%\end{minipage}
%\hfill
%%
%\begin{minipage}[b]{0.49\linewidth}
%\caption{Yellow-red differences overlayed on a patient image. Hopefully showing good stuff..}
%\label{fig:Differences}
%\end{minipage}
%\end{figure}

%Specifically, we train our model on half of the healthy subjects, and predict scans for patient diagnosed with AD. We also predict scans for a held-out set of healthy subjects, and as expected, we estimate warps more accurately for healthy subjects than for those diagnosed with AD (Fig.~\ref{fid:application}). Futhermore, we compare the areas of the brain anatomy that differ in the predicted healthy brain of a subject with AD diagnosis and observe changes relevant to AD, such as shrinkage of the ventricles. 


%We illustrate a representative predicted image in Fig.~\ref{fig:validation} and see that our model predicts plausible images.

==> MICCAI2015 - arxiv2020/experiments_.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{./figures/volumeerror}
\caption{Relative error (lower is better) of volume prediction for seven structures for high-change subjects (top decile of volume change). For each structure, we show relative error between the baseline and the follow-up measurement, relative error in prediction using a linear model, and relative error in prediction using our complete model.}
\label{fig:volumeerror}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.74\linewidth]{./figures/ADvalidation}
\includegraphics[width=0.24\linewidth]{./figures/healthyprediction_135299}
\caption{Prediction results. Left: The Dice scores of labels propagated through three methods for several AD-relevant structures in subjects with the most volume change for each structure. For each structure, we show registration of the baseline to the follow-up image through the atlas as a standard measure, and the registrations predicted by our model and the simplified linear regression model. Right: A predicted anatomical image for a patient diagnosed with AD using a healthy model, showing significant shrinkage of the ventricles when compared to the observed follow-up.}
\label{fig:ADDice}
\end{figure}

\section{Experiments}
We illustrate preliminary prediction results through three separate experiments that use genetic, clinical and imaging data from the ADNI longitudinal cohort~\cite{jack2008}. Subjects have two to ten follow-up scans covering~$0.5 - 7$ years after baseline. We register all scans affinely to a template constructed from~$145$ randomly chosen subjects, and compute registration warps~$\Phi_{AI}$ for each image using ANTs~\cite{avants2011}. For each experiment, we use clinical and genetic data as packaged for the Alzheimer's Disease Big Data DREAM Challenge~\footnote{https://www.synapse.org/\#!Synapse:syn2290704}. Specifically, for each patient we use a list of~$21$ genetic loci, and standard clinical factors including age, gender, marital status, education, disease diagnostic, and cognitive tests. We also make use of pre-computed structure volumes for the ventricles, hippocampus, whole brain volume, entorhinal cortex, fusiform gyrus, middle temporal gyrus and intercranial volume using FreeSurfer~\cite{fischl2012}. For the first two experiments, we learn our model parameters from 341 subjects and predict follow-up volumes on for a separate set of 100 subjects. 

%We also do a simulation study (not shown) and found that our model improves prediction over a standard linear model for non-negligible values of~$\frac{\tau}{\sigma}$. 



\subsection{Volumetric Predictions}
In our first experiment, we predict volume measurements of the available anatomical structures mentioned above. We use our prediction method, as well as a simple linear regression model that does not consider subject-specific health profiles (i.e,~$H=0$). Our model is able to accurately predict volumetric changes. Many subjects do not have dramatic changes in the given structures over time, and our algorithm shows modest improvement over linear regression with an average of~$0.126$ points less percent error. However, when considering the more difficult case of prediction of subjects with large volume changes over time, our model improves prediction dramatically as shown in Fig.~\ref{fig:volumeerror}. 



\subsection{Image Prediction}
Next, we validate our model for full anatomical prediction as described in Section~\ref{sec:appearancemodel}. To generate follow-up images, we predict their warps from the atlas~$\hat{\Phi_{AI_F}}$. We use our model, as well as the simplified linear regression, and compare the results with true warps~$\Phi_{AI_F}$. 

We quantify our results by propagating labels of anatomical structures using our predicted warp. We compare the resulting segmentations to manual labels of follow-up scans via Dice scores for structures relevant to Alzheimer's Disease (AD). As before, our model using appearance phenotypes shows modest improvement of 1.7 dice points compared to the linear model across the entire testing set. Looking at the more difficult predictions in subject with significant change for each structure, we observe large prediction improvements, ranging from 2 to 17 dice points across the different structures.

We note that the anatomical model depends on registration accuracy, which can strongly affect appearance results. In particular, for many scans, the overlap of the labels baseline and the follow-up labels is higher than the composition of registrations from baseline to the follow up through the atlas. A different choice of appearance model may therefore offer improved image prediction, which we leave for future work.



\subsection{Application: Patterns of Disease Progression}
To demonstrate the potential of our anatomical prediction, we predict the follow up scan of a patient diagnosed with dementia as if that patient were healthy. Specifically, we train our model using healthy subjects, and predict scans for patients diagnosed with AD. In Figure~\ref{fig:ADDice} we show an example result, and compare the areas of the brain anatomy that differ in the predicted \textit{healthy} brain of a subject with AD diagnosis. We highlight changes relevant to AD, such as shrinkage of the ventricles. Our prediction therefore illustrates that ventricle shrinkage would be different if this patient had a healthy trajectory.




==> MICCAI2015 - arxiv2020/instantiation.tex <==
\section{Model Instantiation for Anatomical Predictions}
The full model~\eqref{eq:finalychange} can be used with many reasonable phenotype definitions. Here, we describe the phenotype model we use for anatomical predictions and specify the similarity kernels of the health profile.

\subsection{Anatomical Phenotype}
\label{sec:appearancemodel}

We define a voxel-wise phenotype that enables us to predict entire anatomical images.  Let~$\Omega$ be the set of all spatial locations~$v$ (voxels) in an image, and~$I_b = \{I_b(v)\}_{v\in\Omega}$ be the acquired baseline image. We similarly define~$A = \{A(v)\}_{v\in\Omega}$, to be the population atlas template. We assume each image~$I$ is generated through a deformation field~$\Phi_{AI}^{-1}$ parametrized by the corresponding displacements~$\{\bu(v)\}_{v\in\Omega}$ from the common atlas to the subject-specific coordinate frame~\cite{rohlfing2009}, such that~$
	%A_x \rightarrow I_x + \Phi_x.
	%I_x = \Phi_x^{-1}(A_x) \\
	I(v) = A(v + \bu(v)).
$
%
We further define a follow-up image~$I_t$ as a deformation~$\Phi_{Bt}$ from the baseline image~$I_b$, which can be composed to yield an overall deformation from the atlas to the follow-up scan via~$\Phi^{-1}_{At}=\Phi^{-1}_{AB} \circ \Phi^{-1}_{Bt} = \{\bu'(v)\}_{v\in\Omega}$:
%
\begin{align}
	%A_x \rightarrow I_x + \Phi_x.
	%I_b(v) &\rightarrow I_t(v) + \bu'(v) \\
	%A(v) \rightarrow I_b(v) + \bu(v) &\rightarrow I_t(v) + (\bu(v) + \bu'(v))
%	I'_x = \Phi_x^{'-1}(A_x) = (\Phi_x \circ \Delta \Phi_x)(A_x).
%
%	I_B(v) \rightarrow I_t(v + u'(v)) \\
%	A(v) = I_B(v + u(v)) \\
%	A(v) = I_t(v + u(v) + u'(w))
	I_t(v) = A(v + \bu'(v)).
\end{align}
%

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/anatomical_prediction_overview}
	\caption{Overview of anatomical prediction. Arrows represent a displacement vector at each voxel from the common atlas space to the subject space. We predict the change in a displacement field from the baseline (orange) to the follow-up timepoint (purple) using external factors. A follow-up image can then be formed by propagating voxels from the baseline, to the atlas, and finally to the follow-up image locations.}
	\label{fig:schematic_anatomicalprediction}
\end{figure}

Using displacements~$\bu'(v)$ as the phenotype of interest in~\eqref{eq:pred} captures the necessary information for predicting new images, but leads to very high dimensional descriptors. To regularize the transformation and to improve efficiency, we define a low-dimensional embedding of~$\bu'(v)$. Specifically, we assume that the atlas provides a parcellation of the space into L anatomical labels~$\mathcal{L} = \{\Psi\}_{l=1}^L$. We build a low-dimensional embedding of the transformation vectors~$\bu(v)$ within each label using PCA. We define the relevant phenotypes~$\{y_{l,c}\}$ as the coefficients associated with the first~$C$ principal components of the model that capture 95\% of the variance in each label, for~$l=1\ldots L$.

We predict the phenotypes using~\eqref{eq:finalypred}. To construct a follow-up image~$I_t$ given phenotype~$y_t$, we first form a deformation field~$\widehat{\Phi}_{At}^{-1}$ by reconstruction from the estimated phenotype~$y_t$, and use~$\widehat{\Phi}_{At}$ assuming an invertible transformation. Using the baseline image, we predict a subsequent image via~$\Phi_{Bt} = \widehat{\Phi}_{At}\circ\Phi^{-1}_{AB}$. Note that we do not directly model changes in image intensity. While population models necessitate capturing such changes, we predict changes from a baseline image. We also assume that affine transformations are not part of the deformations of interest, and thus all images are affinely registered to the atlas. %, and all follow-up images affinely registered to their respective baselines.

Using this appearance model, we use equation~\eqref{eq:finalypred} to predict the anatomical appearance at every voxel, as illustrated in Figure~\ref{fig:schematic_anatomicalprediction}.

\subsection{Health Similarities}
To fully define the health similarity term~$H(\cdot, \cdot, \cdot)$, we need to specify the forms of the kernel functions~$K_G(\cdot, \cdot)$,~$K_C(\cdot, \cdot)$, and~$K_I(\cdot, \cdot)$.

For genetic data, we employ the identical by state (IBS) kernel often used in genetic analysis~\cite{queller1989}. Given a vector of genetic variants~$\bg$ of length~$S$, each genetic locus is encoded as~$\bg(s) \in \{0, 1, 2\}$, and
%indicates the number of nucleotides that match the most frequent nucleotide in the population (major allele) at that location. The IBS kernel is then defined as
%

\begin{equation}
	K_G(\bg_i, \bg_j) = \frac{1}{2S} \sum_{s=1}^S (2-|\bg_i(s) - \bg_{j}(s)|).
\end{equation}
%

To capture similarity of clinical indicators~$\bc$, we  %form the weighted vector~$\bc'(s)= \bw(s) \bc(s)$, where the weights~$\bw$ 
form the kernel function
%

\begin{equation}
	K_C(\bc_i, \bc_j) = \exp \left( -\frac{1}{\sigma^2_C}  (\bc_i - \bc_j)^T\bW(\bc_i - \bc_j) \right),
\end{equation}
%
where diagonal weight matrix~$\bW$ captures the effect size of each clinical indicator on the phenotype, and~$\sigma^2_C$ is the variance of the clinical factors. 

We define the image feature vectors $f_b$ as the set of all PCA coefficients defined above for the baseline image. We define the image kernel matrix as 
%
\begin{equation}
	K_I(f_{b,i}, f_{b,j}) = \exp \left( -\frac{1}{\sigma^2_I}  ||f_{b,i} - f_{b,j}||^2_2 \right),
\end{equation}
%
where~$\sigma^2_I$ is the variance of the image features. 


We emphasize that other data sources can easily be incorporated in the model by simply adding appropriate kernels for that data. 


==> MICCAI2015 - arxiv2020/intro.tex <==
\section{Introduction}

We present a method for predicting anatomy based on external information, including genetic and clinical indicators. Specifically, given only a single baseline scan of a new subject in a longitudinal study, our model predicts anatomical changes and generates a subsequent image by leveraging subject-specific genetic and clinical information. Such voxel-wise prediction opens up several new areas of analysis, enabling novel investigations both at the voxel level and at the level of derivative biomarker measures. For example, voxel level differences between the true progression of a patient with dementia and their predicted healthy anatomy highlight spatial patterns of disease. We validate our method by comparing measurements of volumes of anatomical structures based on predicted images to those extracted from the acquired scans.

Our model describes the change from a single (or \textit{baseline}) medical scan in terms of population trends and subject-specific external information. 
%The first scan of a subject in a longitudinal study serves as the baseline for the purposes of prediction.} 
We model how anatomical appearance changes with age on average in a population, as well as deviations from the population average using a person's \textit{health profile}. We characterize such profiles non-parametrically based on the genotype, clinical information, and the baseline image. Subject-specific change is constructed from the similarity of health profiles in the cohort, using a Gaussian process parametrized by a population health covariance. Given the predicted change, we synthesize new images through an appearance model.

Statistical population analysis is one of the central topics in medical image computing. The classical correlation-based analysis has yielded important characterization of relationships within imaging data and with independent clinical variables~\cite{davis2010,misra2009,Pfefferbaum2013,rohlfing2009}. Regression models of object appearance have been previously used for atlas construction and population analysis~\cite{davis2010,rohlfing2009}. These methods characterize population trends with respect to external variables, such as age or gender, and construct clinically relevant population averages. 

Longitudinal analyses also characterize subject-specific temporal effects, usually in terms of changes in the biomarkers of interest. Longitudinal cohorts and studies promise to provide crucial insights into aging and disease~\cite{misra2009,Pfefferbaum2013}.
%However, prior work in this area typically involve {\color{red}statistical comparisons methods}, and do not attempt to predict relevant features. 
Mixed effects models have been shown to improve estimation of subject-specific longitudinal trends by using inter-population similarity~\cite{durrleman2013,sadeghi2013}. 
While these approaches offer a powerful basis for analysis of biomarkers or images in a population, they require multiple observations for any subject, and do not aim to provide subject-specific predictions given a single observation. The parameters of the models are examined for potential scientific insight, but they are not tested for predictive power.

Recently, several papers have proposed prediction of medical images or specific anatomical structures by extrapolating at least two time points (e.g. a baseline and a follow-up image) to simulate a later follow-up measurement~\cite{blanc2012,fleishman2015}. These models, however, necessitate observations of at least two time points to make predictions which are difficult to acquire for every new patient. They are therefore not applicable to most patients, not applicable during a first visit, and are sensitive to noise in these few measurements. Recent methods have also used stratified population average deformations to make follow-up predictions from a baseline image~\cite{modat2014}. While classified by population subgroups, these predictions are not adapted to a particular subject's health or environment. %In contrast, we use external factors that are learned from a population to make robust predictions. 

%
%Several methods aim to predict population trends for specific biomarkers of shape models, but these studies do not address subject-specific predictions, nor do they predict full anatomical appearance~\cite{blanc2012,?}. 
%
In contrast, we define the problem of population analysis as predicting anatomical changes for individual subjects. Our generative model incorporates a population trend and uses subject-specific genetic and clinical information, along with the baseline image, to generate subsequent anatomical images. This prediction-oriented approach provides avenues for novel analysis, as illustrated by our experimental results. %We are able to predict full subsequent anatomical images, facilitating novel analyses.

%\begin{align}
%	\tau^2_G \\
%	\tau^2_C \\
%	\tau^2_I \\
%	\bK_G \\
%	\bK_C \\
%	\bK_I \\
%	y \\
%	y_0 \\
%	\beta \\
%	\sigma^2 \\
%	I	
%\end{align}

% PREDICTION OF SHAPES KINDA HAPPENS - see Blanc et al, Statistical model based shape prediction from a combination of direct observations and various surrogates: Application to orthopaedic research
%[not generalized ...]

%{\color{red} Our formulation leads to a mixed model? Highlight diffs from mixed models?}

%Many studies have analyzed relationships of anatomical features with clinical factors, and have demonstrated significant correlations. We demonstrate a model that takes advantage of the relationships to achieve prediction of anatomical appearance.





==> MICCAI2015 - arxiv2020/model.tex <==
\section{Prediction Model}

Given a dataset of patients with longitudinal data, and a single baseline image for a new patient, we predict follow-up anatomical states for the patient. We model anatomy as a phenotype~$y$ that captures the underlying structure of interest. For example,~$y$ can be a low-dimensional descriptor of the anatomy at each voxel. We assume we only have a measurement of our phenotype at baseline~$y_b$ for a new subject. Our goal is to predict the phenotype~$y_t$ at a later time~$t$. We let~$x_t$ be the subject age at time~$t$, and define~$\Delta x_t = x_t - x_b$ and~$\Delta y_t = y_t - y_b$. We model the change in phenotype~$y_t$ using linear regression:
%
\begin{align}
	\Delta y_t = \Delta x_t \beta + \epsilon,
	\label{eq:pred}
\end{align}
%
where~$\beta$ is the subject-specific regression coefficient, and noise~$\epsilon \sim \mathcal{N}(0, \sigma^2)$ is sampled from zero-mean Gaussian distribution with variance~$\sigma^2$.

%In the remainder of this section, we first describe the core of our model that captures the changes in anatomical appearance using the population trend and patient specific information, and then outline the resulting prediction algorithm. In the next section, we describe our particular choice of appearance model for phenotype~$y$ to enable prediction of follow-up scans, and describe the subject-specific health profiles.


%\begin{figure}[t]
%\centering
%\begin{minipage}[t]{0.45\linewidth}
%\includegraphics[width=1\linewidth]{./figures/graphicalmodel}
%\end{minipage}
%\hfill
%%
%\begin{minipage}[b]{0.49\linewidth}
%\caption{A graphical representation of our generative model. Circles indicate random variable and rounded squares represent parameters. The plates indicate replication.~$I$ is the predicted image, and~$y_c$ are the phenotypes that help us determine the image. Phenotypes are affected by~$h$, which are drawn from Gaussian processes and capture among-subject similarity through genetic, clinical and imaging factors.}
%\label{fig:graphicalmodel}
%\end{minipage}
%\end{figure}

\subsection{Subject-Specific Longitudinal Change}
%
To model subject-specific effects, we 
%%
%Generalizing \eqref{eq:pred}, we have
%%
%\begin{align}
%y_t = y_0 + x_t \beta + \epsilon
%\end{align}
%%
%%or equivalently,
%%
%%\begin{align}
%%p(y_i | \beta_i; \sigma, y_i(0)) = \mathcal{N}(y_i; y_i(0) + x_i \beta_i, \sigma).
%%\end{align}
%
define~$\beta = \bar{\beta} + H(\bg,\bc,f_b)$, where~$\bar{\beta}$ is a global regression coefficient shared by the entire population, and~$H$ captures a deviation from this coefficient based on the subject's genetic variants~$g$, clinical information~$c$, and baseline image features~$f_b$.

%where~$\bg$ is a vector of genetic variants of a patient,~$\bc$ is a vector of clinical information, and~$\bf_b$ is the a vector of image-based features from the baseline image of the patient

\begin{figure}[t]
	\centering
	\begin{minipage}[t]{0.35\linewidth}
		\includegraphics[width=1\linewidth]{figures/graphicalmodel}
	\end{minipage}
	\hfill
	%
	\begin{minipage}[b]{0.60\linewidth}
		\caption{A graphical representation of our generative model. Circles indicate random variable and rounded squares represent parameters. The plates indicate replication.~$I$ is the predicted image, and~$y_c$ are the phenotypes that help us determine the image. Phenotypes are affected by~$h$, which are drawn from Gaussian processes and capture among-subject similarity through genetic, clinical and imaging factors.}
		\label{fig:graphicalmodel}
	\end{minipage}
\end{figure}

We assume that patients' genetic variants and clinical indicators affect their anatomical appearance, and that subjects with similar health profiles exhibit similar patterns of anatomical change. %Intuitively we want the current subject's deviation~$H(\cdot)$ to be similar to that in subjects from our dataset with a similar health profile. 
%
We let~$h_G(\cdot)$,~$h_C(\cdot)$,~$h_I(\cdot)$ be functions that capture genetic, clinical and imaging effects on the regression coefficients:
%
\begin{align}
	H(\bg, \bc, \bI_b) = h_G(\bg) + h_C(\bc) + h_I(f_b).
\end{align}
% 
Combining with~\eqref{eq:pred}, we arrive at the full model
%
\begin{align}
	\Delta y_t = \Delta x_t \bar{\beta} + \Delta x_t \big( h_G(\bg) + h_C(\bc) + h_I(f_b) \big) + \epsilon,
	\label{eq:finalychange}
\end{align}
%
%
%using equation~\ref{?}, we can then write
%
%\begin{align}
%p(y_i | h_g(g_i), h_C(c_i), h_I(I_i) ; \beta, \sigma, y_i(0)) = %\mathcal{N}(y_i; \mu_i, \sigma), \\
%\mu_i = y_i(0) + x_i \left( h_g(g_i) + h_C(c_i) + h_I(I_i) \right).
%\end{align}
%
which captures the population trend~$\bar{\beta}$, as well as the subject-specific deviations
%from that trend through the subject-specific health
~$[h_G(\cdot), h_C(\cdot), h_I(\cdot)]$. % {\color{red}We rely on similarities in health profiles to construct a non-parametric predictor}.
Together with a description of an image from phenotype~$y$ in the next section, equations~\eqref{eq:finalychange} and~\eqref{eq:gp} define a generative probabilistic interpretation of our model, which we show graphically in Figure~\ref{fig:graphicalmodel}.

For a longitudinal cohort of~$N$ subjects, we group all~$T_i$ observations for subject~$i$ to form~$\Delta \by_{i} = [y_{i_1}, y_{i_2}, ... y_{i_{T_i}}]$. We then form the global vector~$\Delta \by = [\Delta \by_{1}, \Delta \by_{2}, ..., \Delta \by_{N}]$. We similarly form vectors~$\Delta \bx$,~$\bh_G$,~$\bh_C$,~$\bh_I$,~$\boldsymbol{g}$,~$\boldsymbol{c}$,~$\boldsymbol{f_b}$ and~$\bepsilon$, to build the full regression model:
%
\begin{align}
	%	\by &= \by_0 + \bx \left(\bar{\beta} + H(\bg, \bc, \bI_B) \right) + \bepsilon \nonumber \\
	%	&= \by_0 + \bx \left(\beta + \bh_G(\bg) + \bh_C(\bc) + \bh_I(\bI_B) \right) + \bepsilon \nonumber \\
	\Delta \by &= \Delta \bx \bar{\beta} + \Delta \bx \odot \left(\boldsymbol{h}_G(\boldsymbol{g}) + \bh_C(\boldsymbol{c}) + \bh_I(\boldsymbol{f}_b) \right) + \bepsilon,
	\label{eq:population}
\end{align}
%
%where~$\epsilon\sim\mathcal{N}(\cdot, \mathbf{0}, \sigma^2 \mathbb{I})$ and~$h_P \sim GP\{0,\tau_P^2 \bK_P\}$, for $D \in \{G,C,I\}$.
%
where~$\odot$ is the Hadamard, or element-wise product. This formulation is mathematically equivalent to a General Linear Model (GLM)~\cite{mccullagh1984} in terms of the health profile predictors~$[\boldsymbol{h}_G, \bh_C, \bh_I]$. 

We employ Gaussian process priors to model the health functions:
%
\begin{align}
	h_D(\cdot) \sim GP(\mathbf{0}, \tau_D^2 K_D(\cdot, \cdot)),
	\label{eq:gp}
\end{align}
%
where covariance kernel function~$\tau_D^2 K_D(z_i, z_j)$ captures the similarity between subjects~$i$ and~$j$ using feature vectors~$\bz_i$ and~$\bz_j$ for~$D\in\{G,C,I\}$. We discuss the particular form of~$K(\cdot, \cdot)$ used in the experiments later in the paper. 





\subsection{Learning}

The Bayesian formulation in~\eqref{eq:population} and~\eqref{eq:gp} can be interpreted as a linear mixed effects model (LMM)~\cite{mcculloch2001} or a least squares kernel machine (LSKM) regression model~\cite{ge2015,liu2007}. 
%Linear mixed models have been recently used in population genetics to account for confounding structure. 
We use the LMM interpretation to learn the parameters of our model, and the LSKM interpretation to perform final phenotype predictions. 

Specifically, we treat~$\bar{\beta}$ as the coefficient vector of fixed effects and~$\bh_G, \bh_C$, and~$\bh_I$ as independent random effects. We seek the maximum likelihood estimates of parameters~$\bar{\beta}$ and~$\btheta = (\tau^2_G, \tau^2_C, \tau^2_I, \sigma^2)$ by adapting standard procedures for LMMs~\cite{ge2015,liu2007}. As standard LMM solutions become computationally expensive for thousands of observations, we take advantage of the fact that while the entire genetic and the image phenotype data is large, the use of kernels on baseline data reduces the model size substantially. We obtain intuitive iterative updates 
%
%\begin{align}
%	\theta^{(k+1)} = \theta^{(k)} + \frac{1}{2}\left[\mathcal{I}^{(k)}\right]^{-1}\bR^{(k)}
%\end{align}
%
that project the residuals at each step onto the expected rate of change in likelihood, and
%
%where~$\mathcal{I}^{k+1}_{i,j} = \frac{1}{2}\mathrm{tr}(\bP\bK_i\bP\bK_j)$
%,~$\bR=-\frac{1}{2}\mathrm{tr}(\bP\bK_i) + \frac{1}{2}\by'\bP\bK_i \bP y'$
%,~$\bP=\bV^{-1} - \bV^{-1} \mathbbm{1}\bq^T$
%,~$\bq=((\mathbbm{1}^T\bV^{-1}\mathbbm{1})^{-1}\mathbbm{1}^T\bV^{-1})^T$
%,~$\bV=\sum_D\tau^2_D\bK_D + \sigma^2\mathbb{I}$
%, and~$\by'=(\by - \by_0)\odot([\frac{1}{\bx_1}...\frac{1}{\bx_T}]^T)$. 
update~$\bar{\beta}$ using the best linear unbiased predictor.
%
%\begin{align}
%	\bar{\beta} &= \bq^T\by',
%\end{align}
%
%where ~$\by'=(\Delta \by)\odot([\frac{1}{\Delta \bx_1}...\frac{1}{\Delta \bx_T}]^T)$.

\subsection{Prediction}

Under the LSKM interpretation, the terms~$h(\cdot)$ are estimated by minimizing a penalized squared-error loss function, which leads to the following solution~\cite{ge2015,kimeldorf1971,liu2007,wahba1990}:
%
\begin{align}
	h(z_i) = \sum_{j=1}^N \alpha_j K(\bz_i,\bz_j) \quad \mathrm{or} \quad \bh = \balpha^T \bK
\end{align}
%
for some vector~$\balpha$. Combining with the definitions of the LMM, we estimate coefficients vectors~$\balpha_G,\balpha_C$ and~$\balpha_I$ 
from a linear system of equations that involves our estimates of~$\hat{\beta}$ and~$\mathbf{\theta}$.
%
%%from the following linear system of equations:
%%
%\begin{align}
%\Scale[0.73]{
%\left[ \begin{array}{cccc}
%\bone^T\bone & \bone^T\bK_G & \bone^T\bK_C & \bone^T\bK_I \\
%\bK_G^T\bone & \bK_G^T\bK_G + \frac{\tau_G^2}{\sigma^2}\bK_G^T\bone & \bK_G^T\bK_C & \bK_G^T\bK_I \\
%\bK_C^T\bone & \bK_G^T\bone & \bK_C^T\bK_C + \frac{\tau_C^2}{\sigma^2}\bK_C^T\bone & \bK_C^T\bK_I \\
%\bK_I^T\bone & \bK_I^T\bK_G & \bK_I^T\bone & \bK_I^T\bK_I + \frac{\tau_I^2}{\sigma^2}\bK_I^T\bone \end{array} \right] 
%\left[ \begin{array}{c}
%\bar{\beta} \\
%\balpha_G \\
%\balpha_C \\
%\balpha_I \end{array} \right] 
%= 
%\left[ \begin{array}{c}
%\bone^T\by' \\
%\bK_G^T\by' \\
%\bK_C^T\by' \\
%\bK_I^T\by' \end{array} \right], }
%\end{align}
%%
%where ~$\by'=\Delta \by\odot\left[\frac{1}{\Delta \bx_1}...\frac{1}{\Delta \bx_T}\right]$. 
We can then re-write~\eqref{eq:population} as
%
\begin{align}
	\Delta \by = \Delta \bx \bar{\beta} + \Delta \bx \left(\balpha_G^T \bK_G + \balpha_C^T \bK_C + \balpha_I^T \bK_I  \right)
\end{align}
%
and predict a phenotype at time~$t$ for a new subject~$i$:
\begin{align}
	y_t = y_b + \Delta x_t \left[\bar{\beta} + \sum_{j=1}^N \alpha_{G,j} K_G(\bg_i,\bg_j) + \alpha_{C,j} K_C(\bc_i,\bc_j) + \alpha_{I,j} K_I(f_i,f_j)  \right].
	%	y_t = y_b + \Delta x_t \bar{\beta} + \Delta x_t \sum_{j=1}^N \left( \alpha_{G,j} K_G(\bg_i,\bg_j) + \alpha_{C,j} K_C(\bc_i,\bc_j) + \alpha_{I,j} K_I(f_i,f_j) \right)  .
	\label{eq:finalypred}
\end{align}

%
%Finally, using our appearance model, we use equation~\eqref{eq:phen2img} to predict the anatomical appearance at every voxel.


%Our formulation can be seen as a linear mixed model (with tiny modifications). We use maximum likelihood estimates, using existing literature to update parameters. We omit most of the derivations and just show some updates (if any?). Using these updates parameters, we can form~$\beta_i$, and then~$y_i(t)$ in equation~\eqref{eq:pred}.










==> experiments_.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{./figures/volumeerror}
\caption{Relative error (lower is better) of volume prediction for seven structures for high-change subjects (top decile of volume change). For each structure, we show relative error between the baseline and the follow-up measurement, relative error in prediction using a linear model, and relative error in prediction using our complete model.}
\label{fig:volumeerror}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.74\linewidth]{./figures/ADvalidation}
\includegraphics[width=0.24\linewidth]{./figures/healthyprediction_135299}
\caption{Prediction results. Left: The Dice scores of labels propagated through three methods for several AD-relevant structures in subjects with the most volume change for each structure. For each structure, we show registration of the baseline to the follow-up image through the atlas as a standard measure, and the registrations predicted by our model and the simplified linear regression model. Right: A predicted anatomical image for a patient diagnosed with AD using a healthy model, showing significant shrinkage of the ventricles when compared to the observed follow-up.}
\label{fig:ADDice}
\end{figure}

\section{Experiments}
We illustrate preliminary prediction results through three separate experiments that use genetic, clinical and imaging data from the ADNI longitudinal cohort~\cite{jack2008}. Subjects have two to ten follow-up scans covering~$0.5 - 7$ years after baseline. We register all scans affinely to a template constructed from~$145$ randomly chosen subjects, and compute registration warps~$\Phi_{AI}$ for each image using ANTs~\cite{avants2011}. For each experiment, we use clinical and genetic data as packaged for the Alzheimer's Disease Big Data DREAM Challenge~\footnote{https://www.synapse.org/\#!Synapse:syn2290704}. Specifically, for each patient we use a list of~$21$ genetic loci, and standard clinical factors including age, gender, marital status, education, disease diagnostic, and cognitive tests. We also make use of pre-computed structure volumes for the ventricles, hippocampus, whole brain volume, entorhinal cortex, fusiform gyrus, middle temporal gyrus and intercranial volume using FreeSurfer~\cite{fischl2012}. For the first two experiments, we learn our model parameters from 341 subjects and predict follow-up volumes on for a separate set of 100 subjects. 

%We also do a simulation study (not shown) and found that our model improves prediction over a standard linear model for non-negligible values of~$\frac{\tau}{\sigma}$. 



\subsection{Volumetric Predictions}
In our first experiment, we predict volume measurements of the available anatomical structures mentioned above. We use our prediction method, as well as a simple linear regression model that does not consider subject-specific health profiles (i.e,~$H=0$). Our model is able to accurately predict volumetric changes. Many subjects do not have dramatic changes in the given structures over time, and our algorithm shows modest improvement over linear regression with an average of~$0.126$ points less percent error. However, when considering the more difficult case of prediction of subjects with large volume changes over time, our model improves prediction dramatically as shown in Fig.~\ref{fig:volumeerror}. 



\subsection{Image Prediction}
Next, we validate our model for full anatomical prediction as described in Section~\ref{sec:appearancemodel}. To generate follow-up images, we predict their warps from the atlas~$\hat{\Phi_{AI_F}}$. We use our model, as well as the simplified linear regression, and compare the results with true warps~$\Phi_{AI_F}$. 

We quantify our results by propagating labels of anatomical structures using our predicted warp. We compare the resulting segmentations to manual labels of follow-up scans via Dice scores for structures relevant to Alzheimer's Disease (AD). As before, our model using appearance phenotypes shows modest improvement of 1.7 dice points compared to the linear model across the entire testing set. Looking at the more difficult predictions in subject with significant change for each structure, we observe large prediction improvements, ranging from 2 to 17 dice points across the different structures.

We note that the anatomical model depends on registration accuracy, which can strongly affect appearance results. In particular, for many scans, the overlap of the labels baseline and the follow-up labels is higher than the composition of registrations from baseline to the follow up through the atlas. A different choice of appearance model may therefore offer improved image prediction, which we leave for future work.



\subsection{Application: Patterns of Disease Progression}
To demonstrate the potential of our anatomical prediction, we predict the follow up scan of a patient diagnosed with dementia as if that patient were healthy. Specifically, we train our model using healthy subjects, and predict scans for patients diagnosed with AD. In Figure~\ref{fig:ADDice} we show an example result, and compare the areas of the brain anatomy that differ in the predicted \textit{healthy} brain of a subject with AD diagnosis. We highlight changes relevant to AD, such as shrinkage of the ventricles. Our prediction therefore illustrates that ventricle shrinkage would be different if this patient had a healthy trajectory.



